Scope of Large Language Models for Mining Emerging Opinions in Online Health Discourse

In this paper, we develop an LLM-powered framework for the curation and evaluation of emerging opinion mining in online health communities. We formulate emerging opinion mining as a pairwise stance detection problem between (title, comment) pairs sourced from Reddit, where post titles contain emerging health-related claims on a topic that is not predefined. The claims are either explicitly or implicitly expressed by the user. We detail (i) a method of claim identification -- the task of identifying if a post title contains a claim and (ii) an opinion mining-driven evaluation framework for stance detection using LLMs. We facilitate our exploration by releasing a novel test dataset, Long COVID-Stance, or LC-stance, which can be used to evaluate LLMs on the tasks of claim identification and stance detection in online health communities. Long Covid is an emerging post-COVID disorder with uncertain and complex treatment guidelines, thus making it a suitable use case for our task. LC-Stance contains long COVID treatment related discourse sourced from a Reddit community. Our evaluation shows that GPT-4 significantly outperforms prior works on zero-shot stance detection. We then perform thorough LLM model diagnostics, identifying the role of claim type (i.e. implicit vs explicit claims) and comment length as sources of model error.

==> Prompts.tex <==
\section{Prompts}
\subsection{Task: Claim Identification}

Given a set of post titles, our goal was to find the post titles that contained claims. We used both zero-shot and few-shot prompts as discussed below.

\begin{itemize}
    \item \textbf{ZeroShot:} You are given text input. Identify if the input text makes any claim about medical symptoms/treatment or if it is any random question/information. \\
  If a claim about medical symptoms/treatment is being made, return 'Yes' in response, or if it is any random question/information return 'No'.

  \item \textbf{FewShot:} You are given text input. Identify if the input text makes any claim about medical symptoms/treatment or if it is any random question/information.
  If a claim about medical symptoms/treatment is being made, return 'Yes' in response, or if it is any random question/information return 'No'. Here are a few examples:\\
  \textbf{Input:} Long-Covid prevalence in the US by the Open Medicine Foundation\\
  \textbf{Claim:} No\\
  \textbf{Input:} Treatment of Long-Haul COVID Patients With Off-Label Acyclovir\\
  \textbf{Claim:} Yes\\
  \textbf{Input:} What to do about my job?\\
  \textbf{Claim:} No\\
  \textbf{Input:} New symptom : Skin flushing , feeling really hot \&; feverish\\
  \textbf{Claim:} Yes\\
  \textbf{Input:} begging for some hope\\
  \textbf{Claim:} No\\
  \textbf{Input:} New systematic review that supports Covid vaccination reduces the likelihood, severity, and duration of Long covid\\
  \textbf{Claim:} Yes\\
  \textbf{Input:} High levels of Arsenic in my body, anyone done heavy metal testing during long covid?\\
  \textbf{Claim:} Yes\\
  \textbf{Input:} Any Recommendations on HEPA Air Filters?\\
  \textbf{Claim:} No\\
  \textbf{Input:} Long-Covid research in China\\
  \textbf{Claim:} No\\ 
\end{itemize}



\subsection{Task: Stance Detection}

In this task, we considered a list of (post tile, comment) pairs as the input. For each pair, we aimed to determine the stance of the comment with respect to the corresponding title. We used the following zero-shot, few-shot, and chain-of-thought prompting strategies for our task.


\begin{itemize}
    \item \textbf{Zero-shot:} As it relates to the post title, is the comment in FAVOR, AGAINST or NONE? Just answer FAVOR, AGAINST, or NONE.

    \item \textbf{Few-shot:} As it relates to the post title, is the comment in FAVOR, AGAINST or NONE? Just answer FAVOR, AGAINST, or NONE.\\
\textbf{Title:} Treatment of Long-Haul COVID Patients With Off-Label Acyclovir\\
Comment: Had to take it after surgery, didn't make any effect\\
\textbf{Stance:} Against\\
\textbf{Title:} New study shows Covid is causing Cancer (in young people)\\
\textbf{Comment:} "Simple concept, covid damages and damage = increased risk. Add on constant inflammation from immune dysregulation and that also doesn't help. Viruses cause something *like* 15\% of cancers."\\
\textbf{Stance:} Favor\\
\textbf{Title:} The linkage between MTHFR gene mutation, Anxiety/Depression and Long Covd?\\
\textbf{Comment:} My wife has MTHFR which we are told by our doctor caused us to have so many miscarriages (4 total). She and I both got Covid in December 2022 and recovered quickly with no severe symptoms. I recently started feeling severe LC and she is perfectly normal. Just throwing it out there about our experience.\\
\textbf{Stance:} None\\
\textbf{Title:} New theories of the possible link between Covid shots and tinnitus are emerging
\textbf{Comment:} Oh?? And here I was thinking it was because I went to too many metal concerts with no ear protection. No no no it must be the vaccine.. Interesting..\\
\textbf{Stance:} Against\\
\textbf{Title:} The Latest Promising Long COVID Treatment? Psychedelic Drugs\\
\textbf{Comment:} microdosing seemed to work for me. then I got back on LDN and its barely working, if at all.\\
\textbf{Stance:} Against\\
\textbf{Title:} The linkage between MTHFR gene mutation, Anxiety/Depression and Long Covd?\\
\textbf{Comment:} I found out I have MTHFR, slow COMT, as well as a gene which predisposes me to worse Covid outcomes\\
\textbf{Stance:} Favor\\
\textbf{Title:} Article: Long COVID stemmed from mild cases of COVID-19 in most people, according to a new multicountry study\\
\textbf{Comment:} Well my case was extra mild (no cough, almost no congestion, 3 days of elevated temp 99 to 100), no loss of smell or taste, but the aftermath was way way way worse! As another commenter stated, "mild " is a pretty wide range - anyone who didn't get hospitallized.\\
\textbf{Stance:} Favor\\
\textbf{Title:} Alkaline water improves exercise-induced metabolic acidosis and enhances anaerobic exercise performance in combat sport athletes \\
\textbf{Comment:} Hmm i have my doubts. Im always drinking alkaline water because I have a filter and havent felt any difference at all.\\
\textbf{Stance:} Against\\
\textbf{Title:} New theories of the possible link between Covid shots and tinnitus are emerging\\
\textbf{Comment:} Why are so many people saying this cant be true or that it had to come from being asymptomatic with Covid. Where has common sense gone? Are we not supposed to question things? My gosh, y'all blaming some agenda are the reason why this world is shit. Good forbid if someone doesnt agree with you. Downvotes, calling people names, we dont believe in science, blah blah blah.\\
\textbf{Stance:} None

    \item \textbf{Chain-of-Thought:} As it relates to the post title, is the comment in FAVOR, AGAINST or NONE? Just answer FAVOR, AGAINST, or NONE.\\
\textbf{Title:} Treatment of Long-Haul COVID Patients With Off-Label Acyclovir\\
\textbf{Comment:} Had to take it after surgery, didn't make any effect\\
\textbf{Reason:} The stance of the comment to the title is against as the commentator indicates that Acyclovir had no effect to them after surgery.\\
\textbf{Stance:} Against\\
\textbf{Title:} New study shows Covid is causing Cancer (in young people)\\
\textbf{Comment:} "Simple concept, covid damages and damage = increased risk. Add on constant inflammation from immune dysregulation and that also doesn't help. Viruses cause something *like* 15\% of cancers."\\
\textbf{Reason:} The stance of the comment to the title is Favor as the comment it explains the title further by explaining how covid can cause cancer.\\
\textbf{Stance:} Favor\\
\textbf{Title:} The linkage between MTHFR gene mutation, Anxiety/Depression and Long Covd?\\
\textbf{Comment:} My wife has MTHFR which we are told by our doctor caused us to have so many miscarriages (4 total). She and I both got Covid in December 2022 and recovered quickly with no severe symptoms. I recently started feeling severe LC and she is perfectly normal. Just throwing it out there about our experience.\\
\textbf{Reason:} The stance of the comment to the title is None as the commentor just shares their story and neither agrees of disagrees with the title.\\
\textbf{Stance:} None\\
\textbf{Title:} The Latest Promising Long COVID Treatment? Psychedelic Drugs\\
\textbf{Comment:} microdosing seemed to work for me. then I got back on LDN and its barely working, if at all.\\
\textbf{Reason:} The stance of the comment to the title is Against as the commentor disagrees with the title and says that microdosing helped initially but is not effective later.\\
\textbf{Stance:} Against\\
\textbf{Title:} The linkage between MTHFR gene mutation, Anxiety/Depression and Long Covd?\\
\textbf{Comment:} I found out I have MTHFR, slow COMT, as well as a gene which predisposes me to worse Covid outcomes\\
\textbf{Reason:} The stance of the comment to the title is Favor as the commentor shares that they had MTHFR and that worsened covid condition thereby agreeing with the title.\\
\textbf{Stance:} Favor\\
\textbf{Title:} Article: Long COVID stemmed from mild cases of COVID-19 in most people, according to a new multicountry study\\
\textbf{Comment:} Well my case was extra mild (no cough, almost no congestion, 3 days of elevated temp 99 to 100), no loss of smell or taste, but the aftermath was way way way worse! As another commenter stated, "mild " is a pretty wide range - anyone who didn't get hospitallized.\\
\textbf{Reason:} The stance of the comment to the title is Favor as the commentor exactly agrees with the title and shares that they had mild covid but long covid after was very bad.\\
\textbf{Stance:} Favor\\
\textbf{Title:} Alkaline water improves exercise-induced metabolic acidosis and enhances anaerobic exercise performance in combat sport athletes\\
\textbf{Comment:} Hmm i have my doubts. Im always drinking alkaline water because I have a filter and havent felt any difference at all.\\
\textbf{Reason:} The stance of the comment to the title is Against as the commentor says Alkaline water didn't make any difference.\\
\textbf{Stance:} Against
\end{itemize}



==> sections/0_Abstract.tex <==
Number of pages: \ztotpages\\
\begin{abstract}
To be Added
\end{abstract}


==> sections/10_EthicalConsiderations_BroadImpact.tex <==
\section{Ethics Statement}
All research was conducted under approval from the Institutional Review Board (IRB) at the submitting author's institution. We collect all data from the subreddit r/covidlonghaulers. Reddit was chosen as the data source as it contains anonymous, publicly available user-generated health texts. We ensure that no sample included in LC-Stance contains personally identifying information. To prevent misuse of any user data used in this study, we will require users to sign a data use agreement before accessing LC-Stance. 

A potential negative impact of our dataset is that surfacing conflicting opinions on long COVID treatments may cause anxiety among affected individuals. However, the potential benefits of surfacing such information (e.g., creating awareness, encouraging people to contact a professional healthcare provider, inform public health policy research, etc.) outweigh the potential negative impacts.

==> sections/5_Experiments.tex <==
\section{Experiments}



==> table_figure_tex/tables/analysis.tex <==

\appendix 
\section{Appendix}
\begin{table*}[!ht]
    \footnotesize
    \centering
    \begin{tabular}{p{7cm}|c|ccc|ccc}
    \hline
    & & \multicolumn{3}{|c|}{Ground Truth} & \multicolumn{3}{c}{Model Output} \\
    Post Title (Claim) & Comments & Against & Favor & None & Against & Favor & None  \\
    \hline
    \hline
    New   theories of the possible link between Covid shots and tinnitus are emerging & 36 & 36\%  & 31\%  & 33\% & 22\%  & 39\%  & 39\% \\
    \hline
The Latest Promising Long COVID Treatment? Psychedelic Drugs & 35 & 34\%  & 46\%  & 20\% & 14\%  & 43\%  & 43\% \\
    \hline
Long-Covid prevalence in the US by the Open Medicine Foundation & 16 & 19\%  & 50\%  & 31\% & 19\%  & 38\%  & 44\% \\
    \hline

Article: Long COVID stemmed from mild cases of COVID-19 in most   people, according to a new multicountry study & 14 & 7\%   & 50\%  & 43\% & 14\%  & 64\%  & 21\% \\
    \hline

New study shows Covid is causing Cancer (in young people)  & 14 & 21\%  & 64\%  & 14\% & 29\%  & 50\%  & 21\% \\
    \hline

Treatment of Long-Haul COVID Patients With Off-Label Acyclovir & 13 & 31\%  & 46\%  & 23\% & 25\%  & 25\%  & 50\% \\
    \hline

The linkage between MTHFR gene mutation, Anxiety/Depression and Long Covd?  & 12 & 17\%  & 33\%  & 50\% & 0\%   & 42\%  & 58\% \\
    \hline

Alkaline water improves exercise-induced metabolic acidosis and   enhances anaerobic exercise performance in combat sport athletes  & 3  & 33\%  & 33\%  & 33\% & 33\%  & 0\%   & 67\% \\
    \hline

Tiziana Life Sciences to assess intranasal foralumab for long Covid & 2  & 0\%   & 100\% & 0\%  & 0\%   & 50\%  & 50\% \\
    \hline

``Era Has Passed": Beijing Subway Drops Mandatory Covid Mask Rule & 2  & 100\% & 0\%   & 0\%  & 100\% & 0\%   & 0\%  \\
    \hline

Nicotine rebalances NAD+ homeostasis and improves aging-related symptoms in male mice by enhancing NAMPT activity \- Nature Communications \- NAD+ is central to cellular energy. Explains a lot. & 1  & 0\%   & 100\% & 0\%  & 0\%   & 100\% & 0\% \\
\hline \textbf{Weighted average} & & \textbf{28\%} & \textbf{44\%} & \textbf{28\%} & \textbf{19\%} & \textbf{41\%} & \textbf{39\%} \\ \hline
    \end{tabular}
    \caption{\label{proj2 breakdown} For each post title in our evaluation set, we show the number of top-level comments on the post. We stratify the comments by their ground truth stance and their stance as assigned by the LLM when prompted by our in-context chain-of-thought prompt.}
\end{table*}
